Erasing the Ephemeral: Joint Camera Refinement and Transient Object Removal for Street View Synthesis

Synthesizing novel views for urban environments is crucial for tasks like autonomous driving and virtual tours. Compared to object-level or indoor situations, outdoor settings present unique challenges, such as inconsistency across frames due to moving vehicles and camera pose drift over lengthy sequences. In this paper, we introduce a method that tackles these challenges on view synthesis for outdoor scenarios. We employ a neural point light field scene representation and strategically detect and mask out dynamic objects to reconstruct novel scenes without artifacts. Moreover, we simultaneously optimize camera pose along with the view synthesis process, and thus, we simultaneously refine both elements. Through validation on real-world urban datasets, we demonstrate state-of-the-art results in synthesizing novel views of urban scenes.

==> figures_tex/kitti_novel.tex <==
\begin{figure*}[t!]
\setlength{\tabcolsep}{1pt}
\newcolumntype{Y}{>{\centering\arraybackslash}p{0.19\linewidth}}
\begin{tabular}{YYYYY}
  Reference  & Nerf-W~\cite{nerfw} &  Nope-NeRF~\cite{nopenerf} & NPLF~\cite{ost2022neural}  &  Ours \\
  \includegraphics[width=\linewidth]{example-image-a} & \includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} \\
\includegraphics[width=\linewidth]{example-image-a} & \includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} 
  
  \end{tabular}\label{fig:kitti_recon}
  \caption{Novel view synthesis results on KITTI~\cite{kitti}.}
  \vspace{-0.35cm}
  \end{figure*}

==> figures_tex/kitti_recon.tex <==
\begin{figure*}[t!]
\setlength{\tabcolsep}{1pt}
\newcolumntype{Y}{>{\centering\arraybackslash}p{0.19\linewidth}}
\begin{tabular}{YYYYY}
  Reference  & Nerf-W~\cite{nerfw} &  Nope-NeRF~\cite{nopenerf} & NPLF~\cite{ost2022neural}  &  Ours \\
  \includegraphics[width=\linewidth]{example-image-a} & \includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} \\
\includegraphics[width=\linewidth]{example-image-a} & \includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} &
\includegraphics[width=\linewidth]{example-image-a} 
  
  \end{tabular}\label{fig:kitti_recon}
  \caption{Reconstruction results on KITTI~\cite{kitti}.}
  \vspace{-0.35cm}
  \end{figure*}
